FMint: Bridging Human Designed and Data Pretrained Models for Differential Equation Foundation Model

The fast simulation of dynamical systems is a key challenge in many scientific and engineering applications, such as weather forecasting, disease control, and drug discovery. With the recent success of deep learning, there is increasing interest in using neural networks to solve differential equations in a data-driven manner. However, existing methods are either limited to specific types of differential equations or require large amounts of data for training. This restricts their practicality in many real-world applications, where data is often scarce or expensive to obtain. To address this, we propose a novel multi-modal foundation model, named \textbf{FMint} (\textbf{F}oundation \textbf{M}odel based on \textbf{In}i\textbf{t}ialization), to bridge the gap between human-designed and data-driven models for the fast simulation of dynamical systems. Built on a decoder-only transformer architecture with in-context learning, FMint utilizes both numerical and textual data to learn a universal error correction scheme for dynamical systems, using prompted sequences of coarse solutions from traditional solvers. The model is pre-trained on a corpus of 40K ODEs, and we perform extensive experiments on challenging ODEs that exhibit chaotic behavior and of high dimensionality. Our results demonstrate the effectiveness of the proposed model in terms of both accuracy and efficiency compared to classical numerical solvers, highlighting FMint's potential as a general-purpose solver for dynamical systems. Our approach achieves an accuracy improvement of 1 to 2 orders of magnitude over state-of-the-art dynamical system simulators, and delivers a 5X speedup compared to traditional numerical algorithms. The code for FMint is available at \url{https://github.com/margotyjx/FMint}.

==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
{\bf Neural network for dynamical systems.}
In recent years, neural network-based solvers have been widely applied to scientific problems such as solving ODEs, PDEs, operator learning, and inverse problems. One common approach parameterizes PDE solutions using feed-forward neural networks \citep{han2018solving,han2017deep,karniadakis2021physics,cui2024data,de2023ai,sirignano2018dgm,yu2018deep,YUAN2024Optimalcontrol,wang2024beno}, where physical laws are enforced via hard or soft constraints in the loss function. The Finite Expression Method (FEX) \citep{liang2022finite,song2023finite,song2024finite} offers an interpretable alternative by representing PDE solutions in computer algebra, capturing solution structure with high accuracy. Neural operator learning \citep{li2010fourier,ong2022iae,cao2021choose,li2022transformer,zhang2021mod,lu2021learning} maps varying parameters or initial conditions to solutions, achieving discretization invariance but requiring large amounts of high-quality data and lacking generalization to unseen distributions.

Recent research has explored integrating traditional numerical algorithms with deep learning to improve the accuracy of dynamical system simulations~\citep{guo2022personalized,huang2023fast}. For instance, NeurVec~\citep{huang2023fast} enables rapid ODE simulations with large time steps, achieving decent accuracy on several classic systems. However, its limited generalization to out-of-distribution systems restricts its practicality for large-scale real-world simulations.

{\bf Foundation model in scientific machine learning.}

Large language models like GPT-4~\citep{achiam2023gpt}, DALL-E~\citep{ramesh2021zero}, and Llama~\citep{touvron2023llama} have achieved remarkable success across various domains~\citep{thirunavukarasu2023large,devlin2018bert,sun2024triforce,qin2023tool,hu2024minicpm,li2023compressing,bi2024decoding,jiang2024hummer}, including text-to-visual generation~\citep{ji2024t2vbench,ji2024tltscore} and information retrieval~\citep{kang2024c}. These models leverage extensive pre-training and adapt to downstream tasks via zero-shot or few-shot learning~\citep{wang2024parameter,yu2023visual}, demonstrating impressive transfer learning capabilities. Inspired by these advances, foundation models have gained traction in scientific machine learning. For example, \citet{subramanian2024towards} explored the Fourier Neural Operator (FNO)~\citep{li2010fourier} for solving classical PDEs, while the Unified PDE Solver (UPS)~\citep{shen2024ups} extended this approach to 1D and 2D PDEs using pre-trained models. Additionally, \citet{mccabe2023multiple} embedded PDEs with varying properties into a shared space, and \citet{rahman2024pretraining} enhanced attention mechanisms for handling PDEs with diverse dimensions.

A growing area in scientific machine learning is in-context learning~\citep{dong2022survey,xie2021explanation,olsson2022context,wei2022chain,xu2024can}, where models are prompted with example pairs and trained to predict new queries based on observed patterns. The In-context Operator Network (ICON) \citep{yang2023context,yang2024pde,yang2023prompting} applies this approach to operator learning by leveraging example pairs with varying PDE parameters and solutions to predict solutions for new query data.

==> sections/tables_figures/MAEvsEpoch.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{FMint_exp_fig/MAEvsEPOCH/lorenz_MAE_vsEpoch.pdf}
    \caption{MAE v.s. fine-tuning steps for Lorenz equation.}
    \label{fig:enter-label}
\end{figure}

==> sections/tables_figures/diff_behav_fig.tex <==
\begin{figure}[ht]
    \centering
    % First figure
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{FMint_exp_fig/Diff_behav_demos/Lorenz_oscillatory.pdf}
        \caption{Lorenz - oscillatory}
        \label{fig:Lorenz_oscillatory}
    \end{subfigure}
    % Second figure
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{FMint_exp_fig/Diff_behav_demos/Lorenz_classic_chaotic.pdf}
        \caption{Lorenz - chaotic}
        \label{fig:Lorenz_chaotic}
    \end{subfigure}
    \caption{\footnotesize Figures showing Lorenz attractors' behavior under two different sets of parameters. (a) shows trajectories generated with $\sigma=12.69, \beta=2.59,\rho=24.33$ under two initial conditions $[1,1,1]$ and $[20,20,20]$ for 10000 steps with $\Delta t = 0.004$. (b) shows trajectories generated with $\sigma=12.69, \beta=2.59,\rho=78.06$ under two initial conditions $[1,1,1]$ and $[20,20,20]$ for 10000 steps with $\Delta t = 0.004$.}
    \label{fig:diff_behav_lorenz}
\end{figure}


